Hypergraph Convolutional Networks via Equivalency between Hypergraphs and Undirected Graphs

As a powerful tool for modeling complex relationships, hypergraphs are gaining popularity from the graph learning community. However, commonly used frameworks in deep hypergraph learning focus on hypergraphs with edge-independent vertex weights (EIVWs), without considering hypergraphs with edge-dependent vertex weights (EDVWs) that have more modeling power. To compensate for this, we present General Hypergraph Spectral Convolution (GHSC), a general learning framework that not only handles EDVW and EIVW hypergraphs, but more importantly, enables theoretically explicitly utilizing the existing powerful Graph Convolutional Neural Networks (GCNNs) such that largely ease the design of Hypergraph Neural Networks. In this framework, the graph Laplacian of the given undirected GCNNs is replaced with a unified hypergraph Laplacian that incorporates vertex weight information from a random walk perspective by equating our defined generalized hypergraphs with simple undirected graphs. Extensive experiments from various domains including social network analysis, visual objective classification, and protein learning demonstrate the state-of-the-art performance of the proposed framework.

==> 2_related_work.tex <==
\section{Related Works}
\label{sec:related_work}
 \textbf{Deep learning for hypergraphs.}
Many hypergraph deep learning algorithms can essentially be viewed as redefining hypergraph propagation schemes on equivalent clique graph~\cite{agarwal2006higher} or its variants~\cite{hgnn,hypergcn,dong2020hnhn}. On the other hand, \cite{UniGNN} and \cite{chien2021allset} propose a message-passing and set function learning framework that covers the MPNN~\cite{MPNN} paradigm.
However, these frameworks fail to provide guarantees. Furthermore, they depend on the elaborate design of propagation schemes.
It remains open in deep hypergraph learning are: (i) a framework that can handle EDVW-hypergraphs (ii) a general theoretical framework that can directly utilize the  build on the Laplacian of hypergraph.

\textbf{Graphs Neural Networks.}
GNNs have received significant attention recently and many successful architectures have been raised for various graph learning tasks~\cite{kipf2016semi,MPNN,velivckovic2018graph}. Spectral-based GNNs have a solid foundation in graph
signal processing~\cite{shuman2013emerging} and allow for simple model property analysis. There exist many powerful spectral-based models such as ChebNet~\cite{defferrard2016convolutional}, GCN~\cite{GCN},SSGC~\cite{zhu2021simple}, GCNII~\cite{gcnii}, APPNP~\cite{klicpera2018predict}. Nevertheless, these methods only employ graphs and not hypergraphs. Fortunately, in our framework, these spectral methods can be extended  to hypergraphs.
 
\textbf{Equivalence between hypergraphs and graphs.} A fundamental problem in the spectral theoretical study of hypergraphs is the equivalency with undigraphs. So far, equivalence is established from two perspectives:the spectrum of Laplacian~\citep{agarwal2006higher,hayashi2020hypergraph} or random walk~\citep{2019random}. 
An important application of building up the equivalence between hypergraphs and graphs is to transform hypergraphs to clique graphs~\cite{zhou2006learning,agarwal2006higher,hein2013total,2019random}.

\input{tables/tab_object_all}
\textbf{Hypergraph with edge-dependent vertex weights.}
EDVW-hypergraphs have been widely adopted in  machine learning  applications, including 3D object classification~\citep{zhang2018dynamic}, image segmentation~\citep{ding2010interactive}, e-commerce~\citep{li2018tail}, image search~\citep{huang2010image}, hypergraph clustering~\citep{hayashi2020hypergraph} , text ranking~\cite{bellaachia2013random}, etc. However, the design of deep learning algorithms for processing EDVW-hypergraphs remains an open question.

% Due to the space limit, more discussions on related works are  deferred to Appendix ~\ref{appendix_related_work}.


==> 7_6app-hy-parti.tex <==
 \section{Generalized Hypergraph Partition}\label{app:hypergraph_partition}
 
 For arbitrary vertex subset $S\subset \V$, $S^{c}$ denotes the compliment of $S$. We define the hyperedge boundary $\partial S$ as $\partial S:=\left\{e \in E \mid e \cap S \neq \emptyset, e \cap S^{c} \neq \emptyset\right\}$. We will generalize the hypergraph partition problem in \citet{zhou2006learning} to our unified hypergraph framework. Hypergraph partition is to cut vertex set $\V$ into two parts $S$ and $S^{c}$. As shown in Theorem \ref{Th:EquivalencyDirectgrpah2hypergraph}, we are inspired to adopt the custom of directed graph normalized cut to formulate the hypergraph partition in a mathematical expression. We need to reuse the definition of $\operatorname{vol}( S)$ and $\operatorname{vol} (\partial S)$ for directed graphs as:
 \begin{align*}
    \operatorname{vol}(S) = \sum_{u \in S}\pi({u}),\quad \operatorname{vol}(\partial S) = \sum_{u\in S}\sum_{v\in S^{c}} \pi({u})P({u,v}) 
 \end{align*}
 And the objective function of the hypergraph partition can be expressed as:
 \begin{equation}
\underset{\emptyset \neq S \subset \V}{\operatorname{argmin}}~c(S):=\operatorname{vol} \partial S\left(\frac{1}{\operatorname{vol} (S)}+\frac{1}{\operatorname{vol}( S^{c})}\right) .
\end{equation}
 
 As we need the explicit form of stationary distribution to formulate this problem, we set the unified random walk on a hypergraph that satisfies with the conditions in Thm. \ref{Th:EquivalencyGrpah2Hyeprgrpah}. % $\Q_{1}=\Q_{2}=\Q$.  
 Then we have:
  \begin{align*}
   \operatorname{vol}(S) &= \frac{\sum_{u \in S}\hat d({u})}{\operatorname{vol}(\V)},\\
    \operatorname{vol}(\partial S) &= \frac{1}{\operatorname{vol}(\V)}\sum_{e \in \partial S}\sum_{u\in e\cap S}\sum_{v \in e\cap S^{c}} w(e)\rho(\delta(e))Q_2(u,e)Q_2(v,e)\\
    &=\frac{1}{\operatorname{vol}(\V)}\sum_{e \in \partial S} w(e)\rho(\delta(e))m(e\cap S)m(e\cap S^{c})
 \end{align*}
where  $m(e\cap S) = \sum_{u\in e\cap S}Q_2(u,e)$ is a measure on the subset of $V$ which explicitly demonstrates  the difference between \citet{zhou2006learning}~(where $m(e\cap S) = \sum_{u\in e\cap S}H(u,e)$)  and our work. We considerate more fine-grained information on vertices when we establish a measure on arbitrary subset of $\V$ and involve the degree of hyperedges to impact the corresponding hyperedge weights rather than use the a priori hyperedge weights. 
 

==> 7_8app-nonlazy.tex <==
\section{Unified Non-lazy Random Walks on Hypergraph}\label{appendixSec:non-lazy_random_walk}
The non-lazy version is nontrivial to factor and analyze. To ease the studies, we first give the following definition and lemma.
\begin{definition}[Reversible Markov chain]\label{def:Reverible_markov}
    Let M be a Markov chain with state space $\mcal X$ and transition probabilities $P(u,v)$, for $u, v \in \mcal X $. We say M is
    reversible if there exists a probability distribution $\pi$ over $\mcal X$ such that
    \begin{align}
    \label{Eq:reversible_condition}
        \pi(u)P(u,v) = \pi(v)P(v,u) .   
    \end{align}
\end{definition}
\begin{lemma}[\citet{2019random}]
    \label{Le:markov2undigraph}
    Let $M$ be an irreducible Markov chain with finite state space $\mcal S$ and transition probabilities $P(u,v)$ for $u,v \in \mcal S$. $M$ is reversible if and only if there exists a weighted, undirected graph $\mcal G$ with vertex set $\mcal S$ such that a random walk on $\mcal G$ and $M$ are equivalent.
\end{lemma}
\paragraph{Proof.} Let $\pi$ be the stationary distribution of $M$~(suppose that is irreducible). Note that $\pi(u)\neq 0$ due to the irreducibility of $M$. Let $\G$ be a graph with vertices $\mcal S$. Different from \citet{2019random}, we set the edge weights of $\G$ to be
\begin{align}
    \label{Eq:weights_of_equivelent_undigraph}
    \omega(u,v)=c\pi(u)P(u,v),\quad \forall\ u,v\in \mcal S
\end{align}
where $c>0$ is a  constant for normalizing $\pi$. With reversibility, $\G$ is well-defined~(i.e. $\omega(u,v)=\omega(v,u)$). In a random walk on $\G$, the transition probability from $u$ to  $v$ in one time-step is: 
$\frac{\omega(u,v)}{\sum_{v\in \V}\omega(u,v)}=\frac{c \pi(u)P(u,v)}{\sum_{v\in \V} c\pi(u)P(u,v)}=P(u,v)$, since $\sum_{w\in \mcal S}P(u,w)=1$. 
Thus, if $M$ is reversible, recall Definition \ref{def:equi}, the stated claim holds. The other direction follows from the fact that a random walk on an undirected graph is always reversible (Aldous \& Fill,[70]).


Next, we generalize the non-lazy random walk of \citet{carletti2021random} to our unified non-lazy random walk with vertex weights $\Q_1, \Q_2$.

\begin{definition}[Unified Non-lazy Random Walk on Hypergraphs]\label{def:non_lazy_random_walk}
Suppose  $\delta(e):= \sum_{v\in \V} Q_2(v,e)$ is the degree of hyperedge, and  $d_{nl}(v) := \sum_{e \in \E} w(e)(\delta(e)-Q_2(v,e))\rho(\delta(e)-Q_2(v,e))Q_1(v,e)$ is the degree of vertex $v$.
The unified \emph{non-lazy} random walk on a hypergraph $\mathcal{H}$ is defined in a two-step manner: Given the current vertex $u$, 

   \textbf{Step I}:  choose a hyperedge $e$ incident to $u$, with probability
    \begin{equation}
        p_1 = \frac{w(e) (\delta(e)-Q_2(u,e)) \rho(\delta(e)-Q_2(u,e))Q_1(u,e)}{d_{nl}(u)}; \label{eq:p1_nl}
        \end{equation}
        
        \textbf{Step II}:  choose an arbitrary vertex $v\neq u$ from $e$, with probability  \label{eq:p2_nl}
        \begin{equation}
        p_2=\frac{Q_2(v,e)}{\delta(e)-Q_2(u,e)},    
    \end{equation}
\end{definition}

Thus, the transition probability of our unified non-lazy random walk from vertex $u$ to $v$ is:
 \begin{align}
 \label{Eq:nonlazy_transition probability}
    P_{nl}(u,v)=\left\{\begin{array}{cl}
    \sum_{e \in \E} \frac{w(e)\rho(\delta(e)-Q_2(u,e))Q_1(u,e)Q_2(v,e) }{d_{nl}(u)}& \text{if }  u \neq v,\\
    0 & \text{if } u=v
    \end{array}\right.
\end{align}
Thus, the transition matrix of unified non-lazy random walk can be expressed as:
\begin{equation}
    \P_{nl}=\D_{nl}^{-1}(\Q_1 \odot \rho(\mbf{1}\D_{e}-\Q_2)) \W\Q_2^{\top},    
\end{equation}

where $\D_{nl}$, $\D_e$ are diagonal matrices with entries $D_{nl}(v,v)=d_{nl}(v)$ and $D_e(e,e)=\delta(e)$, respectively. $\odot$ denotes the Hadamard product and $\mbf{1}$ denotes a $|\V|\xx|\E|$ ones matrix(i.e. all elements equal to 1). 
$\rho(\mbf{1}\D_{e}-\Q_2))$ represents the function $\rho$ acting on each element of $(\mbf{1}\D_{e}-\Q_2)$. 

Following \citet{2019random}, the modified version of the clique graph without self-loops is defined below:
\begin{definition}[\citet{2019random}]
    Let $\mcal H(\V,\E,\Q)$ be a hypergraph associated with the unified non-lazy random walk in Definition \ref{def:non_lazy_random_walk}. The clique graph of $\mcal H $ without
self-loops, $\G^{C}_{nl}$, is a weighted, undirected graph with vertex set $\V$ , and edges $\E'$ defined by
\begin{align}
   \E'= \{(v, w) \in \V \xx \V : v, w \in e \text{ for some } e \in \E, \text{ and } v \neq w \}   
\end{align}
 
\end{definition}

Different from the lazy random walk, a unified  non-lazy random walk on a hypergraph with condition (1) or condition (2) in Thm. ~\ref{Th:EquivalencyGrpah2Hyeprgrpah} is
not guaranteed to satisfy reversibility~(see Definition \ref{def:Reverible_markov}). However, if $\Q_1=\Q_2=\H$, then reversibility holds, and we obtain the
result below.

\begin{theorem}
    Let $\mcal H(\V,\E,\Q)$ be a hypergraph associated with the unified non-lazy random walk in Definition \ref{def:non_lazy_random_walk}. Let $\Q_1=\Q_2=\H$, i.e. $Q_i(v,e) = 1,i\in\{1,2\}$ for all vertices $v$ incident hyperedges $e$. Then, there exist weights $\omega(u,v)$ on the clique graph without self-loops $\G^{C}_{nl}$ such that a non-lazy
    random walk on $\mcal H$ is equivalent to a random walk on $\G^{C}_{nl}$.
\end{theorem}

\paragraph{Proof.}
    We first prove that the unified non-lazy random walk on $\mcal H$ is reversible. It is easy to verify the stationary distribution of the unified non-lazy random walk on $\mcal H$ with $\Q_1=\Q_2=\H$ is
    $\pi(v) = \frac{d_{nl}(v)}{\sum_{v\in\V}d_{nl}(v)}$. %for normalizing constant c > 0.
    Let $P(u,v)$ be the probability of going from u to v in a unified non-lazy random walk on
    $\mcal H$, where $u \neq v$. Then,
    \begin{align*}
        \pi(u)P(u,v)&=\frac{d_{nl}(u)}{\sum_{u\in\V}d_{nl}(u)} \sum_{e \in \E} \frac{w(e)\rho(\delta(e)-Q_2(u,e))Q_1(u,e)Q_2(v,e) }{d_{nl}(u)}\\
        &= \frac{1}{\sum_{u\in\V}d_{nl}(u)} \sum_{e \in \E} (w(e)\rho(\delta(e)-Q_2(u,e))Q_1(u,e)Q_2(v,e) ) \\
        & = \frac{1}{\sum_{u\in\V}d_{nl}(u)} \sum_{e \in \E} (w(e)\rho(\delta(e)-H(u,e))H(u,e)H(v,e) ) \\
        & = \frac{1}{\sum_{u\in\V}d_{nl}(u)} \sum_{e \in \E} (w(e)\rho(\delta(e)-H(v,e))H(v,e)H(u,e) ) \\
        &=\pi(v)P(v,u)
    \end{align*}
    
    So the unified non-lazy random walk is reversible. Thus, by Lemma \ref{Le:markov2undigraph}, there exists a graph $\G$ with
    vertex set $\V$ and edge weights 
    $$\omega(u,v)=d_{nl}(u)P(u,v) $$
    such that a random walk on $\G$ and the unified non-lazy random walk on $\mcal H$ is equivalent. The equivalence of the random walks implies that $P(u,v) > 0$ if and only if $\omega(u,v) > 0$, so it follows that $\G$ is the clique graph of $\mcal H$
    without self-loops.

==> 7_9app_digraph.tex <==
%%=============================================== directed Laplacian 

\section{The Relationship between Generalized Hypergraphs and Digraphs}\label{secapp:relationship_hyper2digraph}

In this part, we would like to illustrate that our unified random walk on a hypergraph is always equivalent to a random walk on the weighted directed  clique graph, 
As long as the equivalent conditions are established, the graphs can be viewed as the low-order encoders of hypergraphs, and many machine learning methods of digraphs  could be  easily generalized to hypergraphs.




\citet{2019random}, whose random walk is a special case of our framework with $\rho(\cdot)=(\cdot)^{-1}, \Q_1=\H$, claims that the hypergraph with edge-dependent weights~(i.e. $\Q_2$ is edge-dependent) is equivalent to a directed graph. Here we extend this conclusion to a more general version by the above definition.

\begin{restatable}{theorem}{restathmone}\textbf{(Equivalency between hypergraph and weighted digraph)}
    \label{Th:EquivalencyDirectgrpah2hypergraph}
      Let $\mathcal{H}(\V,\E,\W,\Q_1,\Q_2)$ denote the generalized hypergraph in Definition \ref{def:generalized hypergraph}. 
     There exists a weighted directed clique graph $\G^C$ such that the random walk on $\mcal{H}$ is equivalent to a random walk on $\G^{C}$.
\end{restatable}


Thm. \ref{Th:EquivalencyDirectgrpah2hypergraph} indicates that any hypergraph is equivalent to a digraph under our framework~(Fig.~\ref{fig:hypergraph2graph_connected}) and implies that the existing hypergraph random walks are modeling pairwise relationships~(proof in Appendix \ref{proof:Th:EquivalencyDirectgrpah2hypergraph} ). 

Adopting results of Thm.  \ref{Th:EquivalencyDirectgrpah2hypergraph}, we design the Laplacian for our unified random walk framework and explore its spectral properties.
Thm. \ref{Th:EquivalencyDirectgrpah2hypergraph} says that the unified random walk framework is equivalent to directed graph, so we extend the definition of directed graph Laplacian~\citep{chung2005laplacians} to  obtain the normalized Laplacian matrix as follows.
\begin{corollary}(\textbf{Random Walk-based Hypergraph Laplacian})
\label{def:digraph-lap}
Let $\mathcal{H}(\V,\E,\W,\Q_1,\Q_2)$ be the generalized hypergraph
Let $\P$ be the transition matrix of our random walk framework on $\mcal H$ with stationary distribution $\pi$~(suppose that exists). Let $\mbf \Phi$ be a $|\V|\xx|\V|$ diagonal matrix with $\Phi(v,v)=\pi(v)$. 
The unified random walk-based hypergraph Laplacian matrix $\L_{rw}$ is defined as: 
    \begin{align}
    \label{Eq:digraph-lap}
        \L_{rw} = \I- \frac{\mbf \Phi^{1/2}\P \mbf \Phi^{-1/2}+\mbf \Phi^{-1/2}\P^{\top}\mbf \Phi^{1/2}}{2}.
    \end{align}
\end{corollary}
\vspace{-0mm}
Following~\citet{chung2005laplacians}, it is easy to study many properties based on Rayleigh quotient of $\L_{rw}$, such as positive semi-definite, Cheeger inequality, etc. The Laplacian $\L_{rw}$ has a great expressive power thanks to the comprehensive random walk, which unifies most of existing random walk-based Laplacian variants due to the generalization ability of the framework~(see Appendix \ref{app:special_case_and Laplacian}). 
Note that the distribution $\pi$ is not easy to obtain and do not admit a unitized expression that limits the application of  $\L_{rw}$ in \Eqref{Eq:digraph-lap}. In this paper, we focus on the case when hypergraph is equivalent to undigraph~(Thm. \ref{Th:EquivalencyGrpah2Hyeprgrpah}) and deduce the explicit expression of $\L_{rw}$ (Corollary \ref{Th:stationary_distribution}). 
%%==========================================================================================end

Based on our equivalency Theorem and Lapalacian, we can design directed graph neural networks for generalized hypergraph learning, which we will do as a future work.

==> images/fig_hypergraph2graphDirected.tex <==
\begin{figure*}
    \centering
    \vspace{-2mm}
    \includegraphics[width=1.0\linewidth]{images/hypergraph2graphDirected.pdf}
     \caption{An example of hypergraph and its equivalent weighted directed graph, where $q^i(\cdot)=Q_i(\cdot,e), i\in\{1,2\}$. Here, $\Q_1$ is edge-dependent and $\Q_2$ is edge-independent. The characteristics of the hypergraph are encoded in the weighted incidence matrices~(i.e. vertex weights) $\Q_1, \Q_2$.
    $\W^{C}:=\Q_1\D_e^{-1}\Q_2^{\top}$ denotes the edge-weight matrix of the clique graph  
     and can be viewed as the embedding of high-order relationships.}
    \label{fig:hypergraph2graphDirected}
        \vspace{-4mm}
\end{figure*}

==> images/fig_protein.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.5\linewidth]{images/protein.pdf}
    
    \caption{An expample of edge-dependent vertex weight matrix $\Q$ of protein.}
    \label{fig:proteinQ}
        \vspace{-2mm}
\end{figure*}

==> images/fig_sigma_sensitivity.tex <==
\begin{figure*}[htbp]
\centering
    \subfigure{
    \begin{minipage}[s]{0.3\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{images/sensitivityOf_sigma.pdf}
    \end{minipage}%
    }%
    \quad 
    \subfigure{
    \begin{minipage}[s]{0.3\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{images/sensitivityOf_beta.pdf}
    \end{minipage}%
    }%
    \quad
    \subfigure{
    \begin{minipage}[s]{0.3\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{images/sensitivityOf_alpha.pdf}
    %\caption{fig2}
    \end{minipage}
    }%

\centering

\caption{Test accuracy by varying the hyper-parameters $\sigma$~(left),  $\beta$~(middle) and $\alpha$~(right) of SHSC. }
\label{fig:sensitivity}
\end{figure*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/object_classification.tex <==
%% SOTA
\begin{table*}[thbp]
\def\p{$\pm$} 
\centering
\setlength\tabcolsep{3pt} 
\vspace{-0.0mm}
\caption{Test accuracy on visual object classification. Each model we ran 10 
random seeds and report the mean \p~standard deviation. BOTH means GVCNN+MVCNN, which represents combining the features or structures to generate multi-modal data. }
    \vspace{-2mm}
\scalebox{0.72}{
\begin{tabular}{c|cc|ccccc}
    \toprule 
    \multirow{1}{*} { Datasets }& \multirow{1}{*} { Feature } & Structure  & HGNN & UniGNN & HGAT & GHCN(ours) & SHSC(ours) \\
    \hline
    \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}NTU\end{tabular}} 
    & MVCNN &  MVCNN & 80.11\p0.38  & 75.25$\pm$0.17 & 80.40$\pm$0.47 & 81.37\p0.63  &  \textbf{82.56\p 0.39}  \\
    & GVCNN &  GVCNN  & 84.26\p0.30  & 84.63$\pm$ 0.21 & 84.45$\pm$0.12 & \textbf{85.15\p0.34 } &  83.35\p 0.30  \\
    & BOTH &  BOTH &  83.54\p0.50  & 84.45$\pm$0.40  & 84.05$\pm$0.36 &  84.45\p 0.40  &   \textbf{85.12\p0.25}  \\
    \hline
    \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Model-\\Net40\end{tabular}} 
    & MVCNN       &  MVCNN       & 91.28\p 0.11  & 90.36$\pm$0.10 & 91.29$\pm$0.15 &  91.99\p 0.16            &  \textbf{92.01\p 0.08}  \\
    & GVCNN       &  GVCNN       &  92.53\p0.06  & \textbf{92.88$\pm$0.10} & 92.44$\pm$0.11 & 92.66\p 0.10  & 
    {92.69\p 0.06}    \\
    & BOTH& BOTH  &   {97.15\p0.14}  & 96.69$\pm$0.07 & 96.44$\pm$0.15 & 97.28\p0.15   &  \textbf{97.78\p0.03}    \\
    \bottomrule
\end{tabular}
}
    \vspace{-6mm}
    \label{tab:object_accuracy} 
\end{table*}


==> tables/tab_protein_QA_fold.tex <==

\begin{table}[thbp]
% \begin{wraptable}{r}{1.0\linewidth}% \end{wraptable}
\def\p{$\pm$} 
\setlength\tabcolsep{3pt} %调整列宽
\centering
\vspace{-0mm}
\caption{Comparison of our method to others on protein Quality Assessment task~(CASP12).  At the residue level, we report \textit{Pearson correlation} across all residues of all decoys of all targets~($R$) and \textit{Pearson correlation} across all residues of per decoys and then average all decoys~($R_{decoy}$) with LDDT scores. At the global level, we report \textit{Pearson correlation} across 
all decoys of all targets~($R$) and \textit{Pearson correlation} per target and then average over all targets~($R_{target}$) with GDT$\_$TS scores.}
\vspace{-2mm}
    \scalebox{0.75}{
    \begin{tabular}{l|cc|cc}
        \toprule 
        \multirow{2}{*} { Methods }
        &
          \multicolumn{2}{c|} { GDT$\_$TS } & \multicolumn{2}{c} { LDDT } \\
          
        & $R$  &  $R_{target}$ & $R$ & $R_{decoy}$ \\
      \midrule
        VoroMQA
        ~\cite{VoroMQA} &  - &  0.557  &  -  &  -  \\
        RWplus~
        \cite{RWplus} &  - &  0.313  &  -  &  -   \\
        3D CNN~
        \cite{3DCNN}        & -   &  0.607  &  -  &  -    \\
        AngularQA
         \cite{AngularQA} &  0.651 &  0.439  &  -  &  -   \\
        \cline{1-5}
         HGNN & 0.667  & { 0.582}  & 0.632    &     0.319  \\
         H-GCN &  0.737  &  \textbf{0.609} &   {0.656}  &  0.340     \\
         H-SSGC (ours) &  \textbf{0.760}  &  0.554  &  \textbf{0.678}  &  \textbf{0.449} \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-4mm}
    \label{tab:Protein_QA_fold}    
\end{table}

==> tables/tab_sota.tex <==
\begin{table*}[th]
\def\p{$\pm$} 
\centering
\vspace{-2mm}
\caption{Summary of classificaiton accuracy(\%) results. We report the average test accuracy and its standard deviation over 10 train-test splits. The number in parentheses corresponds to the number of layers of the model. (OOM: our of memory)}
    \vspace{-2mm}
\scalebox{0.78}{
    \begin{tabular}{cc|c|c|c|c|c}
        \toprule 
              \multicolumn{1}{c}{Dataset}& \multicolumn{1}{c}{Architecture} &\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Cora\\ (co-authorship)\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}DBLP\\ (co-authorship)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Cora\\ (co-citation)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Pubmed\\ (co-citation)\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Citeseer\\ (co-citation)\end{tabular}} \\
        \midrule
             MLP\Done & - & 52.02\p1.7 & 78.72\p0.6 & 52.02\p1.7 & 69.86\p1.6 & 55.03\p1.3 \\
             HyperGCN\Done & spectral-based & 60.66\p10.8 & 84.82\p9.7 & 62.35\p9.3& 68.12\p9.7 & 56.94\p6.3 \\
             HGNN\Done & spectral-based & 69.23\p1.6 & 88.55\p0.18 & 55.60\p1.8& 46.41\p0.7 & 38.98\p1.1 \\
             HNHN & message-passing & 63.95\p 2.4 & 84.43\p 0.3& 41.59\p 3.1 & 41.94\p4.7 & 33.60\p 2.1  \\
             HGAT & message-passing & 65.42$\pm$1.5 & OOM &52.21$\pm$3.5 & 46.28$\pm$0.53 & 38.32$\pm$1.5 \\
             UniGNN &message-passing & 75.30\p1.2 & 88.80\p0.2 & 70.10\p1.4 & 74.40\p 1.0& 63.60\p 1.3 \\
        \midrule
            SSGC & spectral-based & 72.04$\pm$1.2 & 88.61$\pm$0.16 &68.79$\pm$2.1  & 74.49$\pm$1.3 & 60.52$\pm$1.7  \\
            GHCN (ours)& spectral-based & 74.79\p0.91 & 89.04\p 0.19 &{ 69.45\p 2.0} &\textbf{ 75.37\p1.2} & 62.67\p1.2 \\
             SHSC (ours)& spectral-based &\textbf{76.05\p 0.75(6)} & \textbf{89.17\p0.21(16)}  & \textbf{70.64\p 1.8 (32)} & 75.08\p 1.1(4) &\textbf{65.14\p 0.97(32)}\\
        \bottomrule
    \end{tabular}
    }
    \vspace{-5mm}
    \label{tab:sota_accuray}    
\end{table*}


==> tables/tab_text_classification.tex <==

\begin{table*}[htbp]
\centering
\caption{summary of the ModelNet40 and NTU datasets}
\renewcommand\tabcolsep{4.0pt} 
\def\p{$\pm$}
\label{tab:text_dataset}
\vspace{-2mm}
\scalebox{0.9}{
    \begin{tabular}{ c|c|c|c|c|c}
    	\toprule
    	& R52 & R8 & MR  & Ohsumed & 20NG  \\
    	\midrule
    	MLP &  &  &  &  &  \\
    	HyperGCN &  &  &  &  &  \\
    	 HGNN & 90.57\p 0.69 & 95.50\p 0.56 & 72.52\p 1.1 & 31.17 \p 2.16  &  \\
    	\hline
    	HGNN+renormalization & 90.72\p0.53 & 95.76\p0.39 & 72.14 \p 1.4  & 31.79 \p 2.05 &  \\
    	&  &  &  &  &  \\
    	\bottomrule
    \end{tabular}
}
\end{table*}
